DNA-SE: Towards Deep Neural-Nets Assisted Semiparametric Estimation

Semiparametric statistics play a pivotal role in a wide range of domains, including but not limited to missing data, causal inference, and transfer learning, to name a few. In many settings, semiparametric theory leads to (nearly) statistically optimal procedures that yet involve numerically solving Fredholm integral equations of the second kind. Traditional numerical methods, such as polynomial or spline approximations, are difficult to scale to multi-dimensional problems. Alternatively, statisticians may choose to approximate the original integral equations by ones with closed-form solutions, resulting in computationally more efficient, but statistically suboptimal or even incorrect procedures. To bridge this gap, we propose a novel framework by formulating the semiparametric estimation problem as a bi-level optimization problem; and then we develop a scalable algorithm called Deep Neural-Nets Assisted Semiparametric Estimation (DNA-SE) by leveraging the universal approximation property of Deep Neural-Nets (DNN) to streamline semiparametric procedures. Through extensive numerical experiments and a real data analysis, we demonstrate the numerical and statistical advantages of $\dnase$ over traditional methods. To the best of our knowledge, we are the first to bring DNN into semiparametric statistics as a numerical solver of integral equations in our proposed general framework.

==> preamble.tex <==
\usepackage[bookmarks, colorlinks=true, plainpages = false, colorlinks=true, citecolor=red, linkcolor=blue, anchorcolor=red, urlcolor=blue]{hyperref}
\usepackage{url}\urlstyle{rm}
\usepackage{amsmath, amsfonts, amsthm, amssymb, bm, bbm, verbatim, dsfont, mathtools, mathrsfs}
\usepackage{color, graphicx, appendix}
\usepackage{etoolbox}
\usepackage{almendra}
\usepackage{authblk}
\usepackage{array}
\usepackage{multirow}
\usepackage{multicol}

\usepackage{float}
\usepackage{pgf,tikz}
\usetikzlibrary{arrows,shapes.arrows,shapes.geometric,shapes.multipart,fit,automata,decorations.pathmorphing,positioning,shapes.swigs}
\tikzset{
	%Define standard arrow tip
	>=stealth',
	%Define style for boxes
	true/.style={
		rectangle,
		draw=black, very thick,
		text width=6.5em,
		minimum height=2em,
		text centered,
		fill=gray, opacity = 0.5},
	punkt/.style={
		rectangle,
		rounded corners,
		draw=black, very thick,
		text width=6.5em,
		minimum height=2em,
		text centered},
	est/.style={
		circle,
		draw=black, very thick,
		text centered},
	shade/.style={
		circle,
		draw=black, very thick, fill=gray!50,
		text centered},
	weight/.style={
		circle,
		draw=black, very thick,
		text width=6.5em,
		minimum height=2em,
		text centered},
	% Define arrow style
	pil/.style={
		->,
		thick,
		shorten <=2pt,
		shorten >=2pt,},
	double/.style={
		<->,
		thick,
		shorten <=2pt,
		shorten >=2pt,},
	dash/.style={
		dashed,
		thick,
		shorten <=2pt,
		shorten >=2pt,},
	dashdouble/.style={
		<->,
		dashed,
		thick,
		shorten <=2pt,
		shorten >=2pt,}
}

\usepackage{tikz-cd}
\makeatletter 
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}

\usepackage{epstopdf}
\usepackage{fullpage}
\usepackage{algorithm}
\usepackage{algorithmicx}
% \usepackage[noend]{algorithmic}
\usepackage{subcaption}

\usepackage[nameinlink]{cleveref}
\usepackage[round]{natbib}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}     % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}
\usepackage{pdfpages}
\usepackage{scalerel}
\usepackage{dashrule}
\usepackage{lmodern}
\usepackage{fancyhdr}
\usepackage{tabu}
\usepackage{enumitem}

\newcommand{\am}[1]{\noindent{\textcolor{blue}{\textbf{\#\#\# AM:} \textsf{#1} \#\#\#}}}
\newcommand{\yb}[1]{\noindent{\textcolor{red}{\textbf{\#\#\# YB:} \textsf{#1} \#\#\#}}}
\newcommand{\sm}[1]{\noindent{\textcolor{orange}{\textbf{\#\#\# SM:} \textsf{#1} \#\#\#}}}

\def\pa{\mathsf{pa}}
\def\de{\mathsf{de}}
\def\ch{\mathsf{ch}}
\def\an{\mathsf{an}}

\def\poly{\mathsf{poly}}
\def\polylog{\mathsf{polylog}}
\def\EIF{\mathsf{EIF}}
\def\NIF{\mathsf{NIF}}
\def\lin{\mathsf{lin}}
\def\IIFF{\mathbb{IF}}
\def\IF{\mathsf{IF}}
\def\Pr{\mathsf{Pr}}
\def\E{\mathsf{E}}

\def\var{\mathsf{var}}
\def\cov{\mathsf{cov}}
\def\Var{\mathsf{Var}}
\def\Cov{\mathsf{Cov}}
\def\lvert{\left\vert}
\def\rvert{\right\vert}
\def\Pois{\mathsf{Pois}}
\def\mse{\mathsf{mse}}
\def\sd{\mathsf{s.d.}}
\def\Holder{\text{H\"{o}lder}}
\def\CI{\mathsf{CI}}
\def\gan{\mathsf{gan}}
\def\Bias{\mathsf{Bias}}
\def\UCB{\mathsf{UCB}}
\def\se{\mathsf{se}}
\def\SE{\mathsf{SE}}
\def\op{\mathsf{op}}
\def\emp{\mathsf{emp}}

\def\zbar{\bar{\sfz}}
\def\vbar{\bar{\sfv}}
\def\zubar{\ubar{\sfz}}
\def\vubar{\ubar{\sfv}}

\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}

\def\docalc{\mathsf{do}}

\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}

\newcommand{\myreferences}{Master.bib}

%\newcommand{\colorball}[1]{\tikz{\draw[fill=#1,draw=#1] (0,0) circle (3.5pt);}}
%\newcommand{\whiteball}{\tikz{\draw[draw=black] (0,0) circle (3.5pt);}}


%\newcommand{\Vertex}{\tikz[scale=0.5]{\draw (0,0) node (zero) [nodedot] {};}}
%\newcommand{\Edge}{\tikz[scale=0.5]{\draw (0,0) node (zero) [nodedot] {} -- (0.5,0) node (zero) [nodedot] {};}}
%\newcommand{\PathThree}{\tikz[scale=0.5]{\draw (0,0) node (zero) [nodedot] {} -- (0.5,0) node (zero) [nodedot] {} -- (1.0,0) node (zero) [nodedot] {};}}
%\newcommand{\PathFour}{\tikz[scale=0.5]{\draw (0,0) node (zero) [nodedot] {} -- (0.5,0) node (zero) [nodedot] {} -- (1.0,0) node (zero) [nodedot] {}-- (1.5,0) node (zero) [nodedot] {};}}
%\newcommand{\DoubleEdge}{\tikz[scale=0.5,baseline=(zero.base)]{\draw (0,0) node (zero) [nodedot] {} -- (0.5,0) node[nodedot] {};\draw (0,0.5) node[nodedot] {} -- (0.5,0.5) node[nodedot] {};}}
%\newcommand{\Square}{\tikz[scale=0.5,baseline=(zero.base)]{\draw (0,0) node (zero) [nodedot] {} -- (0.5,0) node[nodedot] {} -- (0.5,0.5) node[nodedot] {} -- (0,0.5) node[nodedot] {} -- cycle;}}


\usepackage{xr,xspace}
\usepackage{todonotes}
% \usepackage{paralist}

\usepackage{caption,subcaption,soul}
%\usepackage[ruled,vlined]{algorithm2e}
% http://ctan.org/pkg/algorithms
\usepackage{algpseudocode}
%\usepackage{algorithmicx}% http://ctan.org/pkg/algorithms
\makeatletter
\usepackage{romanbar}
%\renewcommand{\ALG@name}{SDP}
%\renewcommand{\listalgorithmname}{List of \ALG@name s}

%%%%% THEOREM STYLE DEFINITIONS
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{observation}{Observation}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{assumption}{Assumption}
\newtheorem{conjecture}{Conjecture}
\newtheorem{problem}{Problem}
\newtheorem{question}{Question}
\newtheorem{remark}{Remark}
\newtheorem{claim}{Claim}
\newtheorem*{remark*}{Remark}


\newenvironment{problemp}[1]
{\renewcommand{\theproblem}{\ref{#1}$'$}%
    \addtocounter{problem}{-1}%
    \begin{problem}}
    {\end{problem}}

% \renewenvironment{compactitem}
% {\begin{itemize}}
% {\end{itemize}}

\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}

\newcommand{\1}[1]{{\mathbf{1}_{\left\{{#1}\right\}}}}
\newcommand{\post}[2]{\begin{center} \includegraphics[width=#2]{#1} \end{center} }
%\newcommand{\Perp}{\perp \! \! \! \perp}
\newcommand{\Perp}{\perp}
\newcommand{\Hyper}{\text{Hypergeometric}}
\newcommand{\argmax}{\arg\max}
\newcommand{\argmin}{\arg\min}
%\newcommand \P[1]{\mathbb{P}[#1]}
\usepackage{algorithm}
\usepackage{algpseudocode}


%% Wu
\usepackage{xspace, prettyref}

% vocabulary for edge orbits
\newcommand{\matching}{\textsf{matching}}
\newcommand{\bridge}{\textsf{bridge}}
\newcommand{\fork}{\textsf{fork}}
\newcommand{\claw}{\textsf{claw}}
\newcommand{\cycle}{\textsf{cycle}}

\newcommand{\Esingle}{\calE_{\rm single}}
\newcommand{\Edouble}{\calE_{\rm double}}
\newcommand{\ex}{\mathrm{ex}}

\newcommand{\id}{\mathrm{id}}
\newcommand{\lcm}{\mathrm{lcm}}
\newcommand{\termI}{\text{(I)}}
\newcommand{\termII}{\text{(II)}}
\newcommand{\termIII}{\text{(III)}}

\newcommand{\sigmae}{\sigma^{\sf E}} % edge permutation
\newcommand{\pie}{\pi^{\sf E}} 
\newcommand{\tpie}{\tpi^{\sf E}} 

%\newcommand{\cycle}{{\textit{cycle}}}
\newcommand{\diverge}{\to\infty}
\newcommand{\eqdistr}{{\stackrel{\rm (d)}{=}}}
\newcommand{\iiddistr}{{\stackrel{\text{\iid}}{\sim}}}
\newcommand{\inddistr}{{\stackrel{\text{ind.}}{\sim}}}
\newcommand{\ones}{\mathbf 1}
\newcommand{\zeros}{\mathbf 0}
\newcommand{\reals}{{\mathbb{R}}}
\newcommand{\integers}{{\mathbb{Z}}}
\newcommand{\naturals}{{\mathbb{N}}}
\newcommand{\rationals}{{\mathbb{Q}}}
\newcommand{\naturalsex}{\overline{\mathbb{N}}}
\newcommand{\symm}{{\mbox{\bf S}}}  % symmetric matrices
\newcommand{\supp}{{\rm supp}}
\newcommand{\eexp}{{\rm e}}
\newcommand{\rexp}[1]{{\rm e}^{#1}}
\newcommand{\Id}{\mathbf{\mathrm{I}}}
\newcommand{\allones}{\mathbf J}
%\newcommand{\zeros}{\mathbf 0}

\newcommand{\diff}{{\mathrm d}}
\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\green}{\color{green!60!black}}
\newcommand{\nbwu}[1]{{\sf\blue[YW: #1]}}
\newcommand{\nb}[1]{{\sf\blue[#1]}}
\newcommand{\nbr}[1]{{\sf\red[#1]}}
\newcommand{\ssy}[1]{{\sf\green[#1]}}
\newcommand{\Expect}{\mathbb{E}}
\newcommand{\expect}[1]{\mathbb{E}\left[ #1 \right]} 
\newcommand{\eexpect}[1]{\mathbb{E}[ #1 ]}
\newcommand{\expects}[2]{\mathbb{E}_{#2}\left[ #1 \right]}
\newcommand{\tExpect}{{\widetilde{\mathbb{E}}}}
%\newcommand{\Prob}{\mathop{\mathbb{P}}}
\newcommand{\Prob}{\mathbb{P}}
\newcommand{\pprob}[1]{ \mathbb{P}\{ #1 \} }
\newcommand{\prob}[1]{ \mathbb{P}\left\{ #1 \right\} }
\newcommand{\tProb}{{\widetilde{\mathbb{P}}}}
\newcommand{\tprob}[1]{{ \tProb\left\{ #1 \right\} }}
\newcommand{\hProb}{\widehat{\mathbb{P}}}
\newcommand{\toprob}{\xrightarrow{\Prob}}
\newcommand{\tolp}[1]{\xrightarrow{L^{#1}}}
\newcommand{\toas}{\xrightarrow{{\rm a.s.}}}
\newcommand{\toae}{\xrightarrow{{\rm a.e.}}}
\newcommand{\todistr}{\xrightarrow{{\rm D}}}
\newcommand{\toweak}{\rightharpoonup}
\newcommand\indep{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}
\def\ci{\perp\!\!\!\perp} 
\def\Var{\mathrm{Var}}
\def\E{\mathbb{E}}
\newcommand{\Bern}{{\rm Bern}}
\newcommand{\Binom}{{\rm Binom}}
\newcommand{\Uniform}{\mathrm{Uniform}}
\newcommand{\Hyp}{{\rm Hyp}}
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\iid}{i.i.d.\xspace}
% for prettyref.sty
\newrefformat{eq}{(\ref{#1})}
\newrefformat{chap}{Chapter~\ref{#1}}
\newrefformat{sec}{Section~\ref{#1}}
\newrefformat{alg}{Algorithm~\ref{#1}}
\newrefformat{fig}{Fig.~\ref{#1}}
\newrefformat{tab}{Table~\ref{#1}}
\newrefformat{rmk}{Remark~\ref{#1}}
\newrefformat{clm}{Claim~\ref{#1}}
\newrefformat{def}{Definition~\ref{#1}}
\newrefformat{cor}{Corollary~\ref{#1}}
\newrefformat{lmm}{Lemma~\ref{#1}}
\newrefformat{prop}{Proposition~\ref{#1}}
\newrefformat{prob}{Problem~\ref{#1}}
\newrefformat{app}{Appendix~\ref{#1}}
\newrefformat{hyp}{Hypothesis~\ref{#1}}
\newrefformat{thm}{Theorem~\ref{#1}}
\newcommand{\ntok}[2]{{#1,\ldots,#2}}
\newcommand{\pth}[1]{\left( #1 \right)}
\newcommand{\qth}[1]{\left[ #1 \right]}
\newcommand{\sth}[1]{\left\{ #1 \right\}}
\newcommand{\bpth}[1]{\Bigg( #1 \Bigg)}
\newcommand{\bqth}[1]{\Bigg[ #1 \Bigg]}
\newcommand{\bsth}[1]{\Bigg\{ #1 \Bigg\}}
\newcommand{\norm}[1]{\|{#1} \|}
\newcommand{\lpnorm}[1]{\left\|{#1} \right\|_{p}}
\newcommand{\linf}[1]{\left\|{#1} \right\|_{\infty}}
\newcommand{\logorm}[2]{\left\|{#1} \right\|_{{#2}}}
\newcommand{\Lploc}[1]{L^{#1}_{\rm loc}}
\newcommand{\hellinger}{d_{\rm H}}
\newcommand{\Fnorm}[1]{\lnorm{#1}{\rm F}}
\newcommand{\fnorm}[1]{\|#1\|_{\rm F}}
% \newcommand{\opnorm}[1]{\lnorm{#1}{\rm op}}
\newcommand{\opnorm}[1]{\left\| #1 \right\|_2}
% inner product
\newcommand{\iprod}[2]{\left \langle #1, #2 \right\rangle}
\newcommand{\Iprod}[2]{\langle #1, #2 \rangle}
% 12/02/2007
\newcommand{\indc}[1]{{\mathbf{1}_{\left\{{#1}\right\}}}}
\newcommand{\Indc}{\mathbf{1}}
\newcommand{\diag}{\mathsf{diag}}
\newcommand{\degr}{\mathsf{deg} }

\newcommand{\dTV}{d_{\rm TV}}
\newcommand{\tb}{\widetilde{b}}
\newcommand{\tr}{\widetilde{r}}
\newcommand{\tc}{\widetilde{c}}
\newcommand{\tu}{{\widetilde{u}}}
\newcommand{\tv}{{\widetilde{v}}}
\newcommand{\tx}{{\widetilde{x}}}
\newcommand{\ty}{{\widetilde{y}}}
\newcommand{\tz}{{\widetilde{z}}}
\newcommand{\tA}{{\widetilde{A}}}
\newcommand{\tB}{{\widetilde{B}}}
\newcommand{\tC}{{\widetilde{C}}}
\newcommand{\tD}{{\widetilde{D}}}
\newcommand{\tE}{{\widetilde{E}}}
\newcommand{\tF}{{\widetilde{F}}}
\newcommand{\tG}{{\widetilde{G}}}
\newcommand{\tH}{{\widetilde{H}}}
\newcommand{\tI}{{\widetilde{I}}}
\newcommand{\tJ}{{\widetilde{J}}}
\newcommand{\tK}{{\widetilde{K}}}
\newcommand{\tL}{{\widetilde{L}}}
\newcommand{\tM}{{\widetilde{M}}}
\newcommand{\tN}{{\widetilde{N}}}
\newcommand{\tO}{{\widetilde{O}}}
\newcommand{\tP}{{\widetilde{P}}}
\newcommand{\tQ}{{\widetilde{Q}}}
\newcommand{\tR}{{\widetilde{R}}}
\newcommand{\tS}{{\widetilde{S}}}
\newcommand{\tT}{{\widetilde{T}}}
\newcommand{\tU}{{\widetilde{U}}}
\newcommand{\tV}{{\widetilde{V}}}
\newcommand{\tW}{{\widetilde{W}}}
\newcommand{\tX}{{\widetilde{X}}}
\newcommand{\tY}{{\widetilde{Y}}}
\newcommand{\tZ}{{\widetilde{Z}}}

\newcommand{\sfa}{{\mathsf{a}}}
\newcommand{\sfb}{{\mathsf{b}}}
\newcommand{\sfc}{{\mathsf{c}}}
\newcommand{\sfd}{{\mathsf{d}}}
\newcommand{\sfe}{{\mathsf{e}}}
\newcommand{\sff}{{\mathsf{f}}}
\newcommand{\sfg}{{\mathsf{g}}}
\newcommand{\sfh}{{\mathsf{h}}}
\newcommand{\sfi}{{\mathsf{i}}}
\newcommand{\sfj}{{\mathsf{j}}}
\newcommand{\sfk}{{\mathsf{k}}}
\newcommand{\sfl}{{\mathsf{l}}}
\newcommand{\sfm}{{\mathsf{m}}}
\newcommand{\sfn}{{\mathsf{n}}}
\newcommand{\sfo}{{\mathsf{o}}}
\newcommand{\sfp}{{\mathsf{p}}}
\newcommand{\sfq}{{\mathsf{q}}}
\newcommand{\sfr}{{\mathsf{r}}}
\newcommand{\sfs}{{\mathsf{s}}}
\newcommand{\sft}{{\mathsf{t}}}
\newcommand{\sfu}{{\mathsf{u}}}
\newcommand{\sfv}{{\mathsf{v}}}
\newcommand{\sfw}{{\mathsf{w}}}
\newcommand{\sfx}{{\mathsf{x}}}
\newcommand{\sfy}{{\mathsf{y}}}
\newcommand{\sfz}{{\mathsf{z}}}
\newcommand{\sfA}{{\mathsf{A}}}
\newcommand{\sfB}{{\mathsf{B}}}
\newcommand{\sfC}{{\mathsf{C}}}
\newcommand{\sfD}{{\mathsf{D}}}
\newcommand{\sfE}{{\mathsf{E}}}
\newcommand{\sfF}{{\mathsf{F}}}
\newcommand{\sfG}{{\mathsf{G}}}
\newcommand{\sfH}{{\mathsf{H}}}
\newcommand{\sfI}{{\mathsf{I}}}
\newcommand{\sfJ}{{\mathsf{J}}}
\newcommand{\sfK}{{\mathsf{K}}}
\newcommand{\sfL}{{\mathsf{L}}}
\newcommand{\sfM}{{\mathsf{M}}}
\newcommand{\sfN}{{\mathsf{N}}}
\newcommand{\sfO}{{\mathsf{O}}}
\newcommand{\sfP}{{\mathsf{P}}}
\newcommand{\sfQ}{{\mathsf{Q}}}
\newcommand{\sfR}{{\mathsf{R}}}
\newcommand{\sfS}{{\mathsf{S}}}
\newcommand{\sfT}{{\mathsf{T}}}
\newcommand{\sfU}{{\mathsf{U}}}
\newcommand{\sfV}{{\mathsf{V}}}
\newcommand{\sfW}{{\mathsf{W}}}
\newcommand{\sfX}{{\mathsf{X}}}
\newcommand{\sfY}{{\mathsf{Y}}}
\newcommand{\sfZ}{{\mathsf{Z}}}

\newcommand{\sfPi}{\mathsf{\Pi}}

\newcommand{\calA}{{\mathcal{A}}}
\newcommand{\calB}{{\mathcal{B}}}
\newcommand{\calC}{{\mathcal{C}}}
\newcommand{\calD}{{\mathcal{D}}}
\newcommand{\calE}{{\mathcal{E}}}
\newcommand{\calF}{{\mathcal{F}}}
\newcommand{\calG}{{\mathcal{G}}}
\newcommand{\calH}{{\mathcal{H}}}
\newcommand{\calI}{{\mathcal{I}}}
\newcommand{\calJ}{{\mathcal{J}}}
\newcommand{\calK}{{\mathcal{K}}}
\newcommand{\calL}{{\mathcal{L}}}
\newcommand{\calM}{{\mathcal{M}}}
\newcommand{\calN}{{\mathcal{N}}}
\newcommand{\calO}{{\mathcal{O}}}
\newcommand{\calP}{{\mathcal{P}}}
\newcommand{\calQ}{{\mathcal{Q}}}
\newcommand{\calR}{{\mathcal{R}}}
\newcommand{\calS}{{\mathcal{S}}}
\newcommand{\calT}{{\mathcal{T}}}
\newcommand{\calU}{{\mathcal{U}}}
\newcommand{\calV}{{\mathcal{V}}}
\newcommand{\calW}{{\mathcal{W}}}
\newcommand{\calX}{{\mathcal{X}}}
\newcommand{\calY}{{\mathcal{Y}}}
\newcommand{\calZ}{{\mathcal{Z}}}
\newcommand{\orbit}{O}

\newcommand{\comp}[1]{{#1^{\rm c}}}
\newcommand{\Leb}{{\rm Leb}}
\newcommand{\Th}{{\rm th}}

\newcommand{\PDS}{{\sf PDS}\xspace}
\newcommand{\PC}{{\sf PC}\xspace}
\newcommand{\BPDS}{{\sf BPDS}\xspace}
\newcommand{\BPC}{{\sf BPC}\xspace}
\newcommand{\DKS}{{\sf DKS}\xspace}
\newcommand{\ML}{{\rm ML}\xspace}
\newcommand{\SDP}{{\rm SDP}\xspace}
\newcommand{\SBM}{{\sf SBM}\xspace}

\newcommand{\ER}{Erd\H{o}s-R\'enyi\xspace}
\def\Multinom{\mathsf{Multinom}}

\def\Primal{\mathsf{P}}
\def\Dual{\mathsf{D}}

\def\TB{\mathsf{TB}}

\newcommand{\Tr}{\mathsf{Tr}}

\renewcommand{\tilde}{\widetilde}
\renewcommand{\hat}{\widehat}
\newcommand{\mmse}{\mathrm{mmse}}

\newcommand{\overlap}{\mathsf{overlap}}
\newcommand{\Api}{A^{\pi}}
\newcommand{\tpi}{{\widetilde{\pi}}}
\newcommand{\hpi}{{\pi'}}
\newcommand{\harmonic}{{h}}
\newcommand{\fixedpoint}{{e_{A\wedge B^{\pi}}(F)}}
\newcommand{\iii}{{i}}

\newcommand{\stepa}[1]{\overset{\rm (a)}{#1}}
\newcommand{\stepb}[1]{\overset{\rm (b)}{#1}}
\newcommand{\stepc}[1]{\overset{\rm (c)}{#1}}
\newcommand{\stepd}[1]{\overset{\rm (d)}{#1}}
\newcommand{\stepe}[1]{\overset{\rm (e)}{#1}}
\def\alg{\mathsf{alg}}
\def\reg{\mathsf{regret}}

\newcommand{\bma}{{\bm{a}}}
\newcommand{\bmb}{{\bm{b}}}
\newcommand{\bmc}{{\bm{c}}}
\newcommand{\bmd}{{\bm{d}}}
\newcommand{\bme}{{\bm{e}}}
\newcommand{\bmf}{{\bm{f}}}
\newcommand{\bmg}{{\bm{g}}}
\newcommand{\bmh}{{\bm{h}}}
\newcommand{\bmi}{{\bm{i}}}
\newcommand{\bmj}{{\bm{j}}}
\newcommand{\bmk}{{\bm{k}}}
\newcommand{\bml}{{\bm{l}}}
\newcommand{\bmm}{{\bm{m}}}
\newcommand{\bmn}{{\bm{n}}}
\newcommand{\bmo}{{\bm{o}}}
\newcommand{\bmp}{{\bm{p}}}
\newcommand{\bmq}{{\bm{q}}}
\newcommand{\bmr}{{\bm{r}}}
\newcommand{\bms}{{\bm{s}}}
\newcommand{\bmt}{{\bm{t}}}
\newcommand{\bmu}{{\bm{u}}}
\newcommand{\bmv}{{\bm{v}}}
\newcommand{\bmw}{{\bm{w}}}
\newcommand{\bmx}{{\bm{x}}}
\newcommand{\bmy}{{\bm{y}}}
\newcommand{\bmz}{{\bm{z}}}

\newcommand{\bmA}{{\bm{A}}}
\newcommand{\bmB}{{\bm{B}}}
\newcommand{\bmC}{{\bm{C}}}
\newcommand{\bmD}{{\bm{D}}}
\newcommand{\bmE}{{\bm{E}}}
\newcommand{\bmF}{{\bm{F}}}
\newcommand{\bmG}{{\bm{G}}}
\newcommand{\bmH}{{\bm{H}}}
\newcommand{\bmI}{{\bm{I}}}
\newcommand{\bmJ}{{\bm{J}}}
\newcommand{\bmK}{{\bm{K}}}
\newcommand{\bmL}{{\bm{L}}}
\newcommand{\bmM}{{\bm{M}}}
\newcommand{\bmN}{{\bm{N}}}
\newcommand{\bmO}{{\bm{O}}}
\newcommand{\bmP}{{\bm{P}}}
\newcommand{\bmQ}{{\bm{Q}}}
\newcommand{\bmR}{{\bm{R}}}
\newcommand{\bmS}{{\bm{S}}}
\newcommand{\bmT}{{\bm{T}}}
\newcommand{\bmU}{{\bm{U}}}
\newcommand{\bmV}{{\bm{V}}}
\newcommand{\bmW}{{\bm{W}}}
\newcommand{\bmX}{{\bm{X}}}
\newcommand{\bmY}{{\bm{Y}}}
\newcommand{\bmZ}{{\bm{Z}}}

\newcommand{\bba}{{\mathbb{a}}}
\newcommand{\bbb}{{\mathbb{b}}}
\newcommand{\bbc}{{\mathbb{c}}}
\newcommand{\bbd}{{\mathbb{d}}}
\newcommand{\bbe}{{\mathbb{e}}}
\newcommand{\bbf}{{\mathbb{f}}}
\newcommand{\bbg}{{\mathbb{g}}}
\newcommand{\bbh}{{\mathbb{h}}}
\newcommand{\bbi}{{\mathbb{i}}}
\newcommand{\bbj}{{\mathbb{j}}}
\newcommand{\bbk}{{\mathbb{k}}}
\newcommand{\bbl}{{\mathbb{l}}}
\newcommand{\bbm}{{\mathbb{m}}}
\newcommand{\bbn}{{\mathbb{n}}}
\newcommand{\bbo}{{\mathbb{o}}}
\newcommand{\bbp}{{\mathbb{p}}}
\newcommand{\bbq}{{\mathbb{q}}}
\newcommand{\bbr}{{\mathbb{r}}}
\newcommand{\bbs}{{\mathbb{s}}}
\newcommand{\bbt}{{\mathbb{t}}}
\newcommand{\bbu}{{\mathbb{u}}}
\newcommand{\bbv}{{\mathbb{v}}}
\newcommand{\bbw}{{\mathbb{w}}}
\newcommand{\bbx}{{\mathbb{x}}}
\newcommand{\bby}{{\mathbb{y}}}
\newcommand{\bbz}{{\mathbb{z}}}

\newcommand{\bbA}{{\mathbb{A}}}
\newcommand{\bbB}{{\mathbb{B}}}
\newcommand{\bbC}{{\mathbb{C}}}
\newcommand{\bbD}{{\mathbb{D}}}
\newcommand{\bbE}{{\mathbb{E}}}
\newcommand{\bbF}{{\mathbb{F}}}
\newcommand{\bbG}{{\mathbb{G}}}
\newcommand{\bbH}{{\mathbb{H}}}
\newcommand{\bbI}{{\mathbb{I}}}
\newcommand{\bbJ}{{\mathbb{J}}}
\newcommand{\bbK}{{\mathbb{K}}}
\newcommand{\bbL}{{\mathbb{L}}}
\newcommand{\bbM}{{\mathbb{M}}}
\newcommand{\bbN}{{\mathbb{N}}}
\newcommand{\bbO}{{\mathbb{O}}}
\newcommand{\bbP}{{\mathbb{P}}}
\newcommand{\bbQ}{{\mathbb{Q}}}
\newcommand{\bbR}{{\mathbb{R}}}
\newcommand{\bbS}{{\mathbb{S}}}
\newcommand{\bbT}{{\mathbb{T}}}
\newcommand{\bbU}{{\mathbb{U}}}
\newcommand{\bbV}{{\mathbb{V}}}
\newcommand{\bbW}{{\mathbb{W}}}
\newcommand{\bbX}{{\mathbb{X}}}
\newcommand{\bbY}{{\mathbb{Y}}}
\newcommand{\bbZ}{{\mathbb{Z}}}

\newcommand{\sfzbar}{\bar{\sfz}}
\newcommand{\sfvbar}{\bar{\sfv}}
\newcommand{\sfZbar}{\bar{\sfZ}}
\newcommand{\sfVbar}{\bar{\sfV}}

\newcommand{\metric}{\text{\almendra{d}}}

\newcommand{\piML}{\hat{\pi}_{\sf ML}}

\newcommand{\dis}{\mathsf{dis}}
\newcommand{\pre}{\mathsf{pre}}
\newcommand{\nd}{\mathsf{nd}}
\newcommand{\mb}{\mathsf{mb}}
\newcommand{\mpillow}{\mathsf{mp}}
\usepackage{tcolorbox}
\newcommand{\opt}{\mathsf{opt}}

\newcommand{\CATE}{\mathsf{CATE}}

\def\Diag{\mathsf{Diag}}

\def\infl{\mathsf{if}}

\def\proj{\text{proj}}
\def\Holderr{\text{H\"{o}lder}_{r}}

\makeatletter
\def\ubar#1{\underline{\sbox\tw@{#1}\dp\tw@\z@\box\tw@}}
\makeatother

\newcommand*\mycirc[1]{%
\begin{tikzpicture}[baseline=(C.base)]
\node[draw,circle,inner sep=1pt,minimum size=1ex](C) {#1};
\end{tikzpicture}}
